Z-Magic: Zero-shot Multiple Attributes Guided Image Creator

The customization of multiple attributes has gained popularity with the rising demand for personalized content creation. Despite promising empirical results, the contextual coherence between different attributes has been largely overlooked. In this paper, we argue that subsequent attributes should follow the multivariable conditional distribution introduced by former attribute creation. In light of this, we reformulate multi-attribute creation from a conditional probability theory perspective and tackle the challenging zero-shot setting. By explicitly modeling the dependencies between attributes, we further enhance the coherence of generated images across diverse attribute combinations. Furthermore, we identify connections between multi-attribute customization and multi-task learning, effectively addressing the high computing cost encountered in multi-attribute synthesis. Extensive experiments demonstrate that Z-Magic outperforms existing models in zero-shot image generation, with broad implications for AI-driven design and creative applications.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/2_preliminary.tex <==
\label{sec:preliminary}

\section{Preliminaries}
Score-based diffusion models \cite{Hyvarinen05, SongGSE19, 0011SKKEP21, SongDME21}, as a unifying framework, consolidate previous methodologies in both score-based generative modeling and diffusion probabilistic modeling. These models describe the forward diffusion process $\{\mathbf{x}(t)\}_{t=0}^T$ as a stochastic differential equation (SDE). Given this forward SDE, the reverse process can be formulated by solving the corresponding reverse-time SDE in the context of controlled generation \cite{Anderson1982ReversetimeDE, 0011SKKEP21}:
\begin{align}
\label{eq_sde}
    d\mathbf{x} =\Big\{ \mathbf{f}(\mathbf{x}, t) - g(t)^2 &\big[ \nabla_{\mathbf{x}} \log p_t(\mathbf{x}) + \\
    &\nabla_{\mathbf{x}} \log p_t(\mathbf{c} | \mathbf{x}) \big] \Big\} dt + g(t) d\mathbf{\bar{w}}. \nonumber
\end{align}
where $\mathbf{f}(\mathbf{x}, t)$ denotes the drift coefficient, and $\mathbf{\bar{w}}$ represents the standard Wiener process for reverse-time dynamics. Additionally, \cite{0011SKKEP21} proposes a time-dependent score-based model, $\mathbf{s}_{\boldsymbol{\theta}^*}$, to approximate $\nabla_{\mathbf{x}_{t}}\log p(\mathbf{x}_{t})$, thereby enabling the construction and numerical solution of the reverse-time SDE. Our subsequent discussion focuses on the discretization of these stochastic dynamics.


==> sec/intro_back.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{./fig/insight.pdf}
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \includegraphics[width=\linewidth]{./fig/cos_sim_comparison.pdf}
    %     \caption{Gradient Cosine Similarity Variation Across Time-reverse Iterations}
    %     \label{fig:cos_sim_comparison}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.22\textwidth}
    %     \includegraphics[width=\linewidth]{./fig/orth_grad.png}
    %     \caption{Vanilla Gradient Direction}
    %     \label{fig:orth_grad}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.22\textwidth}
    %     \includegraphics[width=\linewidth]{./fig/obtuse_grad.png}
    %     \caption{Ours Gradient Direction}
    %     \label{fig:obtuse_grad}
    % \end{subfigure}
    \caption{We visualize the cosine similarity between gradients introduced by two conditions (i.e., landmark $g_0$ and face ID $g_1$) during the diffusion process. In the vanilla setting, each condition is applied separately without considering contextual coherence, causing the gradient directions to be nearly orthogonal, as random vectors in high-dimensional space are often orthogonal. In contrast, our method adjusts each condition based on the preceding ones, resulting in an obtuse-angled optimization direction where later conditions refine the gradients of earlier ones. In other words, our approach has two degrees of freedom to construct the gradient direction: angle and length.}
    \label{fig:grad}
\end{figure}

With the booming development of generative AI, particularly in the popularization of image generation applications, the paradigm of controlled image creation has garnered significant attention from both the industry and the image synthesis community~\cite{RombachBLEO22, PodellELBDMPR24, RameshPGGVRCS21, abs-2204-06125}.
Under such circumstances, guiding the image creation process via multimodal conditions, encompassing text prompts and reference images, has elicited substantial interest.
The crux of this lies in the capacity to exert effective control over the outcomes of image generation, thereby facilitating customized image creation in line with the anticipated attribute specifications. 

While existing diffusion-based approaches have achieved impressive results in conditional generation~\cite{ZhangRA23, KimODKS24, ChoiKJGY21, HuangC0023, BansalCSSGGG24, 0007DRGM24, AvrahamiHGGTPLF23, HertzVFC24}, underlying structure that inherently links multiple attributes within a coherent creation has been rarely discussed.
In reality, conditional dependence is a fundamental property in multi-attribute guided creation. 
For example, in fashion design, the selection of a color scheme is often influenced by the style or cut of the clothing, and vice versa; similarly, in face synthesis, the presence of gender implies facial features, and this contextual information should guide subsequent attribute choices. 
These examples intuitively illustrate that attributes do not exist in isolation; rather, they are mutually informative and conditionally dependent, forming a naturally coherent whole. 

As shown in Figure~\ref{fig:grad}, another key finding from our experiments reveals a limitation in conventional models: when each attribute is generated independently under the assumption of conditional independence, the conditional gradients associated with different attributes exhibit nearly zero cosine similarity. Mathematically, for any two conditional gradients  $g_{\mathbf{c}_0}$  and  $g_{\mathbf{c}_1}$  during the diffusion process, we observe that  $\mathbb{E}\left[\frac{g_{\mathbf{c}_0}^T g_{\mathbf{c}_1}}{||g_{\mathbf{c}_0}|| ||g_{\mathbf{c}_1}||}\right] \approx 0$, mirroring the behavior of two random high-dimensional vectors \footnote{In high-dimensional spaces, two random vectors are almost always very close to orthogonal.}. 
This outcome is counterintuitive, as these conditions are applied to the same image and, ideally, should exhibit contextual correlation to achieve a harmonious and coherent synthesis. 

In this work, we present a novel approach that explicitly models this conditional dependence, ensuring that each attribute is generated in the context of previously selected ones. 
Specifically, our method utilizes a conditional distribution framework, where each subsequent attribute follows a multivariable conditional distribution informed by the attributes generated before it. 
To realize this, we leverage a score-based conditional diffusion model to control attribute generation. 
Our method is grounded in the gradient-based formulation  $g_{\mathbf{c}} = \nabla_{\mathbf{x}_t} \log p(\mathbf{c} | \mathbf{x}_t)$, where the gradient $g_{\mathbf{c}}$ serves as a means of conditioning, allowing us to refine each attribute based on the context provided by prior attributes.



Instead, we propose a sequential conditioning framework that respects the joint distribution  $p(\mathbf{c}_0, \mathbf{c}_1 | \mathbf{x}_t) $, where each conditionally dependent gradient refines the image generation progressively. Specifically, we apply  $g_0 = \nabla_{\mathbf{x}_t}\log p(\mathbf{c}_0 | \mathbf{x}_t)$  to capture the initial attribute’s influence, followed by  $g_1 = \nabla_{\mathbf{x}_t}\log p(\mathbf{c}_1 | \mathbf{c}_0, \mathbf{x}_t) $, which adjusts the generation to align with the first attribute’s context. As shown in Figure \ref{fig:obtuse_grad}, this sequential conditioning introduces a gradient refinement mechanism where  $g_1$ partially aligns with and corrects the vector length along the  $g_0$  direction, enhancing attribute coherence.

Further, while models can be fine-tuned for specific attribute combinations, training-based approach is resource-intensive and lacks scalability, particularly in the face of high-dimensional attribute spaces. Thus, exploring methods for zero-shot multi-attribute synthesis has the potential to unlock new avenues for practical AI-driven creative tools. In response to these challenges, we introduce Zero-shot Multiple Attributes Guided Image Creator (Z-Magic), an approach designed to address the complex requirements of multi-attribute customization. By reformulating multi-attribute synthesis as a problem of conditional dependency across attributes, Z-Magic leverages principles from conditional probability and multi-task learning to generate coherent images without extensive attribute-specific tuning. This approach not only reduces human labeling overhead for attribute combinations but also paves the way for harmonious customization across diverse domains.





